Nonlinear Modal Reduction for Subwavelength Dielectric Scattering

We study three-dimensional wave scattering by high-index dielectric resonators with Kerr-type nonlinearity under plane-wave incidence, together with the associated nonlinear dielectric scattering resonances, through a nonlinear Lippmann-Schwinger equation. Using a Lyapunov-Schmidt reduction near a simple eigenmode of the Newtonian potential, we obtain a local decomposition of the scattered wave into a resonant contribution and a controlled remainder and derive an explicit nonlinear equation for the resonant modal coefficient for sufficiently small contrast parameter and locally small resonant amplitude and incident field. A second reduction covers the regime of incident fields of order one and weak nonlinearity. Our results extend for the first time the linear modal decomposition to nonlinear wave-scattering problems. We complement them by developing a numerical framework based on Nystr\"om discretization, real Newton iteration, and pseudo-arclength continuation. For single resonators of several geometries, our computations confirm the predicted high-contrast resonance scaling and the nonlinear modal approximation, and exhibit the multivalued incident-wave response. For a mirror-symmetric resonator dimer, we track symmetric, antisymmetric, and symmetry-broken resonance branches over a broad range of separations. Our computations show that the symmetry-breaking threshold increases as the gap between the resonators decreases, in agreement with the leading-order bifurcation theory.

==> macros.tex <==
%macros

% Load packages
\RequirePackage{amsmath,amssymb,amsthm,graphicx,mathrsfs,url, subcaption, listings}
\RequirePackage[usenames,dvipsnames]{color}
\RequirePackage[colorlinks=true,linkcolor=BrickRed,citecolor=RoyalBlue,urlcolor=RoyalBlue]{hyperref}
\RequirePackage{amsxtra}




% Page setup
\setlength{\textheight}{8.50in} \setlength{\oddsidemargin}{0.00in}
\setlength{\evensidemargin}{0.00in} \setlength{\textwidth}{6.08in}
\setlength{\topmargin}{0.00in} \setlength{\headheight}{0.18in}
\setlength{\marginparwidth}{1.0in}
\setlength{\abovedisplayskip}{0.2in}
\setlength{\belowdisplayskip}{0.2in}
% \setlength{\parskip}{0.05in}
% \renewcommand{\baselinestretch}{1.10}

% Include all pictures as MetaPOST
\DeclareGraphicsRule{*}{mps}{*}{}

% change colors for links, visible also for colorblind people
\usepackage{xcolor}
\def\tmp#1#2#3{%
  \definecolor{Hy#1color}{#2}{#3}%
  \hypersetup{#1color=Hy#1color}}
\tmp{link}{HTML}{800006}
\tmp{cite}{HTML}{2E7E2A}
\tmp{file}{HTML}{131877}
\tmp{url} {HTML}{8A0087}
\tmp{menu}{HTML}{727500}
\tmp{run} {HTML}{137776}
% \tmp{note}{HTML}{8A0087}
\def\tmp#1#2{%
  \colorlet{Hy#1bordercolor}{Hy#1color#2}%
  \hypersetup{#1bordercolor=Hy#1bordercolor}}
\tmp{link}{!60!white}
\tmp{cite}{!60!white}
\tmp{file}{!60!white}
\tmp{url} {!60!white}
% \tmp{note}{!60!white}
\tmp{menu}{!60!white}
\tmp{run} {!60!white}


% Equation numbering
\numberwithin{equation}{section}

% arXiv bibliography macro
\def\arXiv#1{\href{http://arxiv.org/abs/#1}{arXiv:#1}}



% Theorems
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}[proposition]{Definition}
\newtheorem{lemma}[proposition]{Lemma}
\newtheorem{corollary}[proposition]{Corollary}
\newtheorem{conjecture}[proposition]{Conjecture}
\newtheorem{question}[proposition]{Question}
\newtheorem{assumption}[theorem]{Assumption}

%% Remark environment changed so font inside is normal
% \theorembodyfont{\normalfont} %needs ntheorem package
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}

% special characters
\newcommand{\C}{\mathbb{C}}
% \newcommand{\K}{\mathbb{K}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\X}{\mathbb{X}}

\newcommand\restrict[1]{\raisebox{-.5ex}{$|$}_{#1}}
% new imaginary unit command
\newcommand{\iu}{{i\mkern1mu}}

%% Use the alternative epsilon per default and define the old one as \oldepsilon
\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\ensuremath\varepsilon}

\let\phi\varphi

\renewcommand{\innerproduct}[2]{\langle #1, #2 \rangle}

% fct definition with 2 lines conditioned - needs amsmath pkg
\newcommand{\twopartdef}[4]{%
\begin{cases}
\displaystyle #1 & \text{if } #2 \\
\displaystyle #3 & \text{if } #4
\end{cases}%
}

% Math operators
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\comp}{comp}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\nbhd}{nbhd}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\Ell}{ell}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\even}{even}
\DeclareMathOperator{\Graph}{Gr}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\HS}{HS}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Imag}{Im}
\let\Im=\Imag % sorry Knuth
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\Op}{Op}
\DeclareMathOperator{\PSL}{PSL}
\DeclareMathOperator{\PSO}{PSO}
\DeclareMathOperator{\Real}{Re}
\let\Re=\Real % sorry Knuth
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\TR}{TR}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\WF}{WF}

\def\WFh{\WF_h}
\def\CIc{C^\infty_{\mathrm{c}}}



\newcommand\subsetsim{\mathrel{%
  \ooalign{\raise0.2ex\hbox{$\subset$}\cr\hidewidth\raise-0.8ex\hbox{\scalebox{0.9}{$\sim$}}\hidewidth\cr}}}


\endinput
